Hardness of Finding Kings and Strong Kings

A king in a directed graph is a vertex $v$ such that every other vertex is reachable from $v$ via a path of length at most $2$. It is well known that every tournament (a complete graph where each edge has a direction) has at least one king. Our contributions in this work are: - We show that the query complexity of determining existence of a king in arbitrary $n$-vertex digraphs is $\Theta(n^2)$. This is in stark contrast to the case where the input is a tournament, where Shen, Sheng, and Wu [SICOMP'03] showed that a king can be found in $O(n^{3/2})$ queries. - In an attempt to increase the "fairness" in the definition of tournament winners, Ho and Chang [IPL'03] defined a strong king to be a king $k$ such that, for every $v$ that dominates $k$, the number of length-$2$ paths from $k$ to $v$ is strictly larger than the number of length-$2$ paths from $v$ to $k$. We show that the query complexity of finding a strong king in a tournament is $\Theta(n^2)$. This answers a question of Biswas, Jayapaul, Raman, and Satti [DAM'22] in the negative. A key component in our proofs is the design of specific tournaments where every vertex is a king, and analyzing certain properties of these tournaments. We feel these constructions and properties are independently interesting and may lead to more interesting results about tournament solutions.

==> Figures/construction-d-imp.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]
    \node[shape=rectangle, minimum size=1em, fill=white,draw=black, minimum size=2cm] (2p) at (1.5,0){$\,\,\,\,\,T[V\setminus\{a,b,c\}]\,\,\,\,\,$};
    \draw[-{Triangle[width=18pt,length=15pt]}, line width=8pt] (1.5,4) to (2p);
    \draw[-{Triangle[width=18pt,length=15pt]}, line width=8pt] (0,3) to (2p);
    \draw[-{Triangle[width=18pt,length=15pt]}, line width=8pt] (3,3) to (2p);
    \node[shape=circle,rounded corners, fill=white, draw=black, minimum size=6mm] (b) at (0,3){$b$};
    \node[shape=circle,rounded corners, fill=white, draw=black, minimum size=6mm] (a) at (1.5,4){$a$};
    \node[shape=circle,rounded corners, fill=white, draw=black, minimum size=6mm] (c) at (3,3){$c$};
    \draw[>=Triangle, ->, ultra thick] (a) to (b);
    \draw[>=Triangle, ->, ultra thick] (b) to (c);
    \draw[>=Triangle, ->, ultra thick] (c) to (a);
\end{tikzpicture}
\vspace{0.5em}
